Moving Forward: A Review of Autonomous Driving Software and Hardware Systems

With their potential to significantly reduce traffic accidents, enhance road safety, optimize traffic flow, and decrease congestion, autonomous driving systems are a major focus of research and development in recent years. Beyond these immediate benefits, they offer long-term advantages in promoting sustainable transportation by reducing emissions and fuel consumption. Achieving a high level of autonomy across diverse conditions requires a comprehensive understanding of the environment. This is accomplished by processing data from sensors such as cameras, radars, and LiDARs through a software stack that relies heavily on machine learning algorithms. These ML models demand significant computational resources and involve large-scale data movement, presenting challenges for hardware to execute them efficiently and at high speed. In this survey, we first outline and highlight the key components of self-driving systems, covering input sensors, commonly used datasets, simulation platforms, and the software architecture. We then explore the underlying hardware platforms that support the execution of these software systems. By presenting a comprehensive view of autonomous driving systems and their increasing demands, particularly for higher levels of autonomy, we analyze the performance and efficiency of scaled-up off-the-shelf GPU/CPU-based systems, emphasizing the challenges within the computational components. Through examples showcasing the diverse computational and memory requirements in the software stack, we demonstrate how more specialized hardware and processing closer to memory can enable more efficient execution with lower latency. Finally, based on current trends and future demands, we conclude by speculating what a future hardware platform for autonomous driving might look like.

==> 06_Potential_Accelerators.tex <==
\section{Deep Learning Hardware Accelerators}
To increase computation efficiency, the incorporation of hardware acceleration into the current self-driving systems is imperative. 


\subsection{Neural Processing Units}

\textcolor{red}{*** This is a new section - need to add new text in here, can use Tesla FSD as a sample ***}


\begin{table*}[ht]
    \centering
        \caption{FPGA-based Accelerators}
    \begin{tabular}{c|c|c|c|c|c|c}
    \hline
    \textbf{Accelerator}  & \textbf{Application} & \textbf{Benchmark} & \textbf{FPS} & \textbf{Frequency (MHz)}  & \textbf{Power (W)} & \textbf{Dataset} \\ \hline
     Wang et. al. \cite{Wang2021FPGAIO}   & Object detection  & YOLOv3  & 84.5 & 300 &  25 &  PASCAL VOC 2007       \\ 
     Nguyen et. al. \cite{Nguyen2019AHA}   & Object detection   & YOLOv2 & 109.3 & 200 & 18.29 & PASCAL VOC 2007 \\ 
     Fang et. al. \cite{Fang2018RealTimeOD} & Object detection    & SSD & 103 &   333 & 11.1 &  -  \\
     Nakahara et. al. \cite{Nakahara2017AnOD} & Object detection & VGG11 BCNN & 34.9 & 200 & 2.5 & KITTI  \\
     Zhan et. al. \cite{Zhan2019LaneDI} & Lane detection  & - & 104 & 100 & - & CIFAR-10       \\ 
          
     Fang et. al \cite{Fang2018RealTimeOD}    & Semantic Segmentation    &  FPN &  128 & 333 & 14.5 & Cityscapes   \\ 
     eSLAM \cite{Liu2019eSLAMAE} & Localization & RS-BRIEF & 55.8 & 100 & 1.94 & TUM dataset\\ 
     \hline
     GPU-based \cite{Wang2021FPGAIO} & Object detection & YOLOv3 & 31.7 & 1607 & 126 & PASCAL VOC 2007  \\
     GPU-based \cite{Redmon2016YOLO9000BF} & Object detection & YOLOv2 & 40-91 & 1000 & 170 & PASCAL VOC 2007  \\
     GPU-based \cite{Fang2018RealTimeOD} & Object detection & SSD & 44.2 & 1480 & 211 & - \\
     GPU-based \cite{Fang2018RealTimeOD} & Semantic Segmentation & FPN & 100 & 1480 & 200 &  Cityscapes \\\hline
     \end{tabular}
    \vspace{0.2cm}

    \label{tab:FPGA_accelerator}
    \vspace{-0.5 cm}
\end{table*}

\subsection{FPGA-based accelerator}
Field Programmable Gates Array (FPGA) offers fine-grained reconfigurability, enabling its implementation of specific calculations in a parallel manner. Therefore, FPGA can be employed to accelerate CPU workloads as FPGA can provide higher parallel compared with traditional CPUs \cite{Dhilleswararao2022EfficientHA} but with a lower frequency. FPGA also provides higher flexibility and shorter development time in contrast to ASIC. Hao et. al. \cite{Hao2019AHG} adopt the FPGA not only as an accelerator but also as a complementary system to increase the overall system reliability of self-driving cars. Sciangula et. al. \cite{Sciangula2022HardwareAO} explored a DNN acceleration shift from GPU-based to FPGA-based in Baidu Apollo self-driving framework. The advantages and challenges are explained for each acceleration strategy. 

In addition to focusing on the acceleration of the whole system, there exist FPGA-based accelerators that target specific tasks, such as object detection. An FPGA-based accelerator was proposed to speed up YOLOv3 for object detection \cite{Wang2021FPGAIO}, resulting in lower power consumption and higher frame rate compared with its GPU counterpart. Nguyen et. al. \cite{Nguyen2019AHA} also accelerated a YOLO CNN on an FPGA platform. Their approach focused on minimizing the access time to off-chip memory, DRAM. This was achieved by optimizing the data path including strategies of data reuse and convolution layers pipeline. As a result of these improvements, access times are reduced, and thus the power efficiency and throughput increase. Fang et. al. \cite{Fang2018RealTimeOD} proposed an architecture, called Aristotle, based on a Xilinx ZU9 FPGA to tackle both object detection and semantic segmentation tasks. A SDD network was adopted to perform the object detection and an FPN was adopted for the semantic segmentation. Nakahara et. al. \cite{Nakahara2017AnOD} designed a BCNN-based accelerator for the object detection task. The accelerator contains a multiscale sliding window part, a BCNN classifier part, and an ARM processing unit. All weights of BCNN were stored in the FPGA on-chip BRAMs and computation units were fully pipelined, resulting in high throughput and lower power implementation.  Zhan et. al. \cite{Zhan2019LaneDI} implemented a lane detection task on an FPGA, resulting in a maximum of 104 FPS. eSLAM \cite{Liu2019eSLAMAE} offers a real-time solution to accelerate the SLAM involved in autonomous localization. It adopts an RS-BREIEF algorithm and implements computation-intensive tasks such as feature extraction and matching on the FPGA. 

The discussed FPGA-based accelerators are summarized in Table \ref{tab:FPGA_accelerator}. This table also includes four GPU implementations to provide a baseline for comparison with GPU acceleration. While the GPUs can provide high frequency, their power consumption is higher than the FPGA. In addition, optimization of data path and exploration of data reuse enables the FPGA-based accelerator to provide a higher throughput, FPS, than their GPU-based counterparts.

Dynamic Random-Access Memory (DRAM), the main memory in a common FPGA board, has limited memory bandwidth and thus may lead to a bottleneck for the whole system, especially when the PEs compute faster than the load data rate. High-bandwidth Memory (HBM) \cite{Lee2015A1V}, enabled by 3D-stacking package technology, provides higher bandwidth than the common DRAM. Utilizing an HBM-based FPGA, Singh et. al. \cite{Singh2021FPGABasedNA} implement the two data-intensive applications, alignment filtering step of genome analysis and representative kernels from the weather prediction model, increasing the performance of energy efficiency and run-time. However, the clock frequency of common FPGA is low and it has a high area usage overhead because of the switching logic to support reconfigurability.

\begin{table*}[ht]
    \centering
        \caption{CGRA-based Accelerators}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline
    \textbf{Accelerator}  & \textbf{Application} & \textbf{Benchmark} & \textbf{GOPS} & \textbf{Freq (MHz)}  & \textbf{Power (W)} & \textbf{Area (mm$^2$)} & \textbf{Process }& \textbf{Dataset} \\ \hline
     EMAX \cite{Tanomoto2015ACA}   & CNN & AlexNet, etc  & 51.2 & 200 &  - &  - & 180 nm  & ImageNet, etc      \\ 

     SDT-CGRA \cite{Fan2018StreamPD} & Object inference & AlexNet, etc & 77.49 & 450 & 77.49  & 5.19 & 55 nm & - \\
     NP-CGRA \cite{Lee2021NPCGRAEC} & DSC & MobileNet-v1& 64 & 500 & - & 2.14 & 65 nm & - \\
     Plasticine \cite{Prabhakar2017PlasticineAR} & CNN, Kmeans & - & 12300 & 1000 & 34.4 & 113 & 28 nm & - \\ \hline
     \end{tabular}
    \vspace{0.2cm}

    \label{tab:CGRA}
    \vspace{-0.5 cm}
\end{table*}


\subsection{CGRA} 
Coarse Grained Reconfigurable Array (CGRA) provides a coarse-grained reconfigurability compared to the FPGA. This architecture typically consists of an array of PEs, which are adept at executing a variety of arithmetic algorithms, and small register files, which store temporary data. Reconfigurable interconnections are integrated between the PEs to support coarse-grained reconfigurability. NeuroCGRA \cite{Jafri2014NeuroCGRAAC} is specifically tailored to enhance support for neural network computation while retaining the functionality of conventional CGRAs. This design is based on Dynamically Reconfigurable Resources Array (DRRA) \cite{Shami2010ControlSF}. EMAX \cite{Tanomoto2015ACA} proposed a CGRA-based architecture with distributed scratchpad memory to reduce the data movement and thus mitigate the bandwidth bottleneck. This architecture is designed to accelerate the CNN. SDT-CGRA \cite{Fan2018StreamPD} is proposed to accelerate the algorithms involved in object detection, such as CNN and Kmeans. To improve the data stream efficiency, it performs a stream-driven execution, increases the intermediate storage space, and adopts both static and dynamic configurations. Furthermore, NP-CGRA \cite{Lee2021NPCGRAEC} focuses on the acceleration of lightweight CNN, such as depthwise separable convolution (DSC), by extending the conventional CGRA architecture and providing a mapping scheme for different types of layers.

While the compilation time of CGRA is typically lower than the FPGA, its compilation time is still considered length compared to traditional CPUs. In addition, traditionally CGRA still requires low-level programming. To address both problems, inspired by the CGRA architectures, Prabhakar et. al. \cite{Prabhakar2017PlasticineAR} propose a parallel-orientated reconfigurable architecture known as Plasticine. This architecture diverges from the traditional approach of using an array composed solely of PEs. Instead, Plasticine employs a memory and compute combined array structure (see figure \ref{fig:Plasticine}) that incorporates the Pattern Compute Units (PCUs), executing different arithmetic algorithms, and Pattern Memory Units (PMUs), storing temporary data for computation and computing the address inside PMU. Switch boxes are integrated to support the connection between different units and address generators (AG) and coalescing units to support communication with a four-channel DRAM. With the foundation of those components, Plasticine can provide superior performance than FPGA. It can support diverse dense applications, such as single precision general matrix multiplication and CNN, and sparse applications, such as sparse matrix-dense vectors and PageRank.

\begin{figure}[htbp]
    \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.485\textwidth]{figures/Plasticine.png}
    \caption{System architecture of Plasticine (actual array size 16 x 8) adopted from \cite{Prabhakar2017PlasticineAR}. PMU: Pattern Memory Unit; PCU: Pattern Compute Unit; AG: Address Generator; S: Switch Box.}
    \label{fig:Plasticine}
    \vspace{-0.2cm}
\end{figure}

Table \ref{tab:CGRA} presents a few CGRA-based accelerators suitable for machine learning applications. Compared to their FPGA counterparts, these accelerators exhibit higher clock frequency as computation units are tailored to specific functions and less area overhead because of fewer interconnections. This specialization, however, results in a reduction of functional flexibility. The computation performance, such as Giga Operation Per Second (GOPS), depends on the available computation units and storage units within the accelerator. Among the discussed accelerators, Plasticine offers the highest computation performance and the highest clock frequency but at the cost of the highest area overhead. Similar to the FPGA-based accelerators, exploration of data reuse and reduction of data movement is also the focus of CGRA-based accelerators.


\begin{table*}[ht]
    \centering
        \caption{ASIC-based Accelerators}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline
    \textbf{Accelerator}  & \textbf{Application} & \textbf{Benchmark} & \textbf{GOPS} & \textbf{Freq (MHz)}  & \textbf{Power (W)} & \textbf{Area (mm$^2$)} & \textbf{Process }& \textbf{Dataset} \\ \hline
     DianNao \cite{Chen2014DianNaoAS}   & CNNs \& DNNs  &  ConvNets & 452 & 980 &  0.485 &  3.02 & 65 nm  & MNIST, etc      \\ 

     ShiDianNao \cite{Du2015ShiDianNaoSV} & CNNs & ConvNN, etc  & 194 & 450 & 0.32  & 4.86 & 65 nm & - \\
     PuDianNao \cite{Liu2015PuDianNaoAP} & DNN, Kmeans, etc & - & 1056 & 500 & 0.596 & 3.51 & 65 nm & MNIST \& UCI data \\
     Eyeriss \cite{Chen2016EyerissAE} & CNNs & AlexNet, etc & 84 & 200 & 0.278 & 12.25 & 65 nm & - \\ 
     Eyerissv2 \cite{Chen2018EyerissVA} & DNNs & MobileNet, etc & 153.6 & 200 & - & - & 65 nm & ImageNet \\ 
     SCNN \cite{Chen2016EyerissAE} & CNNs & AlexNet, etc & 2000 & 1000 & - & 7.9 & 16 nm & - \\ \hline
     \end{tabular}
    \vspace{0.2cm}

    \label{tab:ASIC}
    \vspace{-0.5 cm}
\end{table*}


\subsection{ASIC-based}
Hardware accelerations, when implemented through an Application-Specific Integrated Circuit (ASIC), can be tailored to efficiently execute specific applications but at the cost of flexibility. Therefore they can provide reduced area complexity and power consumption compared to designs based on FPGA and CGRA platforms. Due to their superior energy efficiency and area usage, ASIC-based accelerators are an attractive option in embedded systems or portable devices. Diverse optimizations can be applied \cite{Dhilleswararao2022EfficientHA, Silvano2023ASO} in ASIC-based accelerators, including 1) optimization on the computation unit, arithmetic logic unit (ALU), such as approximate computing paradigm and segmentation method, 2) proper arrangement on the dataflow to reduce the data movement and explore the overlap of activation and weight, 3) sparse computation to avoid useless computation of zero operands.

Convolution is the main computation in neural networks, primarily involving two main mathematical operations: multiplication and addition. This process can be implemented in various structure circuits and optimization can be made to improve their performance. Approximate computing is one of those optimization, which trades the controlled decrease in precision for the sake of improvements in speed and resource efficiency. The output width can be reduced \cite{Jou1999DesignOL}, resulting in a reduced area and delay. Petra et. al. \cite{Petra2010TruncatedBM} introduced a variable-correction truncated multiplier with a compensation function to mitigate the mean square error. Wang et. al. \cite{Wang2011HighAccuracyFM} proposed a fixed-width multiplier with a sorting network-based compensation function to decrease error. Besides approximate computation, the accelerator survey paper \cite{Silvano2023ASO} also mentions convolution optimization and segmentation methods, which can also help to improve the accelerator performance.

\begin{figure}[htbp]
    \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/DianNao.png}
    \caption{Architecture of the DianNao accelerator adopted from \cite{Chen2014DianNaoAS}}
    \label{fig:DianNao}
    \vspace{-0.2cm}
\end{figure}

DianNao \cite{Chen2014DianNaoAS} based on ASIC offers an acceleration solution to the large-scale CNNs and DNNs. It not only focuses on the computation functions but also on the memory behavior, in other words, exploring the data locality to reduce data movement. DianNao architecture is mainly composed of computation units, storage units, and control units. The computation unit, also named the Neural Functional Unit (NFU), is split into two or three stages according to the running layer. Each stage is dedicated to a specific function or computation, such as the NFU-1 stage can be tailored to achieve multiplication functions and the last stage can be customized for non-linear functions. On-chip memory is split into three buffers: an input buffer (NBin), an output buffer (NBout), and a synapse/weight buffer (SB). Dividing buffers can provide benefits to avoid read and write conflicts, which are common challenges in conventional cache systems. In addition, by partitioning buffers, there is an opportunity to explore data reuse. However, DianNao treats the 2D convolution as 1D, making it inefficient for 2D convolution. To address this problem, ShiDianNao \cite{Du2015ShiDianNaoSV} extended the NFU to a 2D Processing Elements (PEs) array. In addition, local storage structures are integrated to facilitate the data movement between PEs, decreasing the DRAM access. Besides supporting neural network-based machine learning (ML) algorithms, PuDianNao \cite{Liu2015PuDianNaoAP} also extends its capability to other ML algorithms, such as Naive Bayes and linear regression. This versatility is achieved by incorporating ALUs and machine learning functional units (MLUs) into PEs.


An efficient dataflow arrangement can provide benefits for exploring data locality in ML networks. The input and output feature maps and the weight can be reused by storing them in the local buffer or scratchpad or utilizing the inter-communication between PEs. Different dataflow models are proposed to explore data reuse and thus reduce data movement. According to \cite{Chen2016EyerissAS}, CNN dataflows can be mainly divided into three types: weight stationary, output stationary, and no local reuse. Eyeriss  \cite{Chen2016EyerissAS, Chen2016EyerissAE} takes all the above reuse into account and can adapt and optimize according to different conditions. A new dataflow model, called row stationary, was proposed to support those functionalities. Eyeriss also supports data compression and sparsity computation to reduce data movement and avoid redundant calculations. It consists of an accelerator connected with an off-chip DRAM (see figure \ref{fig:Eyeriss}). The DRAM provides the input feature map and filters to the accelerator and stores the output feature map from it. The accelerator contains a 12x14 array of PEs, a global buffer, a run-length compression (RLC) decoder and encoder, a ReLU function unit, and network-on-chip (NoC). Each PE is composed of one scratchpad, MAC, and control unit. The global buffer stores the feature maps, filters, and partial sum results. NoC is responsible for the data delivery between the global buffer and PE arrays and between individual PEs. RLC decoder and encoder support the data compression and decompression. respectively. Control units are integrated to manage and direct the traffic among the above function units. With strategies to decrease data movement and improve energy efficiency, Eyeriss can offer 35-frames/s for AlexNet and 0.7-frames/s for VGG-16 with low power consumption. 


\begin{table*}[ht]
    \centering
        \caption{PIM-based Accelerators}
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \hline
    \textbf{Accelerator}  & \textbf{Application} & \textbf{Benchmark} & \textbf{GOPS} & \textbf{Freq (MHz)}  & \textbf{Power (W)} & \textbf{Process} & \textbf{Memory}& \textbf{Location} \\ \hline
     Neurocube \cite{Neurocube}   & Scene Labeling  &  ConvNN & 8 & 300 &  1.86 &  28 nm  & HMC  & Logic layer      \\ 
     Neurocube \cite{Neurocube}   & Scene Labeling  &  ConvNN & 132 & 5000 &  21.5C &  15 nm &  HMC & Logic layer    \\ 
     TETRIS \cite{Gao2017TETRISSA} & DNNs & AlexNet, etc  & - & 500 & 6.94  & 45 nm & HMC & Logic layer \\
     Ambit \cite{Seshadri2017AmbitIA} & Bitwise operations & XOR, AND, etc & - & - & - & 55 nm & HMC & Memory cell  \\
     SIMDRAM \cite{Hajinazar2021SIMDRAMAE} & General operations & VGGNETs, etc & - & - & - & 55 nm & DRAM & Memory cell \\ 
     DrAcc \cite{Deng2018DrAccAD} & CNNs & AlexNet, etc & - & - & 2.5 + $P_{mem}$ & 25 nm & - & Memory cell \\ \hline
     \end{tabular}
    \vspace{0.2cm}

    \label{tab:PIM}
    \vspace{-0.5 cm}
\end{table*}

\begin{figure}[htbp]
    \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/Eyeriss.png}
    \caption{Architecture of Eyeriss accelerator adopted from \cite{Chen2016EyerissAE}}
    \label{fig:Eyeriss}
    \vspace{-0.2cm}
\end{figure}

Input activation and weights in neural networks often include a substantial number of zeros. Multiplication with zero will always result in zero output, resulting in useless computation and power consumption. To tackle this problem, Eyerissv2 \cite{Chen2018EyerissVA} proposed a more coarse-grained accelerator compared to its original version. It integrated an on-chip network (NoC) to adapt different filters and tackle high bandwidth requirements, improving the utilization of resources. The PEs are extended to support sparsity computation and data reuse, increasing energy efficiency and reducing execution time. Compared to its primitive version, Eyerissv2 offers 12.6x faster speed and 2.5x enhancement of energy efficiency for a sparse MobileNet. SCNN \cite{Parashar2017SCNNAA} is an accelerator designed to leverage the data sparsity within the training and inference of CNN. An algorithm dataflow is proposed to enhance data reuse and reduce data movement. AlexNet, GoogLeNet, and VGGNet are evaluated and a maximum of 2 TOPS can be achieved.

The mentioned ASIC-based accelerators are summarized in Table \ref{tab:ASIC}. These accelerators are typically tailored to more specific functions which means lower flexibility compared to their FPGA and CGRA counterparts. However, without the interconnections the accelerator should consume less area usage and low power consumption. Among the presented accelerators, SCNN \cite{Parashar2017SCNNAA} provides the highest throughput and fastest clock speed. Fine-grained circuit design opens up greater opportunities to optimize the critical components of computation units, including multipliers and adders. It also enables the exploration of sparsity computation. Furthermore, optimizing the data flow and integrating minor interconnection circuits can help to improve the functionality and efficiency of ASIC-based accelerators. 



\subsection{Accelerators based on approaching technology}

While the efficient arrangement of the dataflow can help to reduce the data movement thus improving energy efficiency, the bandwidth between the accelerator and off-chip memory, typically DRAM, often remains a bottleneck, especially when the computation unit requires data at a rate faster than the memory can supply. In addition, data movement between the off-chip memory and on-chip is very expensive regarding energy consumption and latency \cite{Boroumand2017LazyPIMAE}. Given these challenges, an interesting question arises: Can we integrate computation directly near or in where data is stored? Theoretical solutions proposed around fifty years ago \cite{Kautz1969CellularLA, Stone1970ALC} centered on a key idea: embedding computation logic within memory. Unfortunately, the adoption of these brilliant ideas has been hindered due to the absence of suitable technologies at that time. Thanks to the advances in 3D-stacked memory technology, new memory standards, such as High-Bandwidth Memory (HBM) and Hybrid Memory Cube (HMC) were proposed. In 3D-stacked memory architecture, multiple memory layers, typical DRAM, are stacked up. Different layers are connected through vertical through-silicon vias (TSVs), enabling high internal bandwidth and throughput. The vertical TSVs also shorten the communication path and thus decrease the delay and energy cost of data movement. 
%3D-stacked memory can also provide more bits of access in parallel than the conventional DRAM, for example, an HBM2 can provide a 4096-bit bus bandwidth in total compared to 256-bit for GDDR5X.
3D-stacked memory can provide higher bandwidth than conventional DDR memory, an HBM from Samsung can provide 1 TB/s bandwidth compared to only 32 GB/s for GDDR5 \cite{HBM2vsDDR5}. 

\begin{figure}[htbp]
    \vspace{-0.2cm}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/TETRIS.png}
    \caption{Architecture of TETRIS accelerator adopted from \cite{Gao2017TETRISSA}, actual array size is 14 x 14}
    \label{fig:TETRIS}
    \vspace{-0.1cm}
\end{figure}




Besides putting the 3D-stacked memory off-chip, the accelerator can be integrated into its logic layer, fully utilizing the high internal bandwidth through the short "wires", vias. Nuerocube \cite{Neurocube} integrates PEs in the logic die of the HMC leveraging the internal high bandwidth to accelerate neural network computation. To achieve fully data-driven computing, programmable neuro sequence generators are associated with vault controllers. Each vault is connected to an individual PE and different PEs communicate through a 2D mesh network. A PE is composed of multiple MACs, a cache memory, a temporal buffer, and a memory module for exploring data reuse with synaptic weights. The Nuerocube accelerator, synthesized at a 15-nm FinFet process, can offer a maximum of 132 GOPS for ConvNN \cite{Gould2009DecomposingAS} inference with a power of 3.41 Watts. TETRIS \cite{Gao2017TETRISSA} is an HMC-based accelerator designed to accelerate DNNs. It integrates the computation array directly into the logic layer of the memory (see figure \ref{fig:TETRIS}), reducing the data movement and increasing the energy efficiency. Each memory stack is divided into sixteen vaults \cite{Jeddeloh2012HybridMC} and each vault contains two DRAM banks. Each vault contains several DRAM banks and a controlling logic connected to them. A DNN accelerator is incorporated in the logic layer by substituting the crossbar network, in the controlling logic, with a 2D mesh NoC. The accelerator architecture is similar to Eyeriss \cite{Chen2016EyerissAE} and is composed of an array of PEs and a global buffer. Each PE contains a small register file and a fixed-point ALU and the global buffer is shared by all the PEs to store temporary data and to support different kinds of data reuse. 

By minor modification of the memory cell of DRAM, simple computation can be implemented just within the memory layers. Ambit \cite{Seshadri2017AmbitIA} supports simple bitwise operations within DRAM by slightly changing the control logic. By simultaneously enabling three rows, bitwise AND and OR operations can be performed. In addition, NOT operation can be achieved by modifying the sense amplifier. The capability to support basic bitwise operation provides the possibility to perform more complex operations, such as XOR operation and even addition and multiplication. SIMDRAM \cite{Hajinazar2021SIMDRAMAE} provides the ability to more efficiently performing complex operations, such as multiplication and addition, compared to Ambit \cite{Seshadri2017AmbitIA}. Complex operations can be decoupled to the majority (MAJ) and NOT operations to improve flexibility by supporting arbitrary operations. To facilitate the implementation of complex operations, a new programming interface, instruction set architecture (ISA) support, and hardware components are integrated. DrAcc \cite{Deng2018DrAccAD}, based on Ambit\cite{Seshadri2017AmbitIA}, incorporates a carry look-ahead adder within the DRAM to accelerate ternary weight neural networks (TWNs). It leverages the basic bitwise operation, AND, OR, and NOT to perform the addition operation. Several circuit modifications are performed to support carry shift and propagation. By utilizing the presented shift and addition circuit, multiplications required by TWN can also be implemented. %Computation units can also be integrated after the bank





==> x02_Sensors_and_Components.tex <==
%\section{Self-Driving System Components}

\section{Sensors and Components} \label{se:sensor, components}
To facilitate self-driving, the ego-vehicle should first efficiently perceive and comprehend its surrounding environment. To tackle these challenges, diverse sensors are fused and integrated into the self-driving systems. Cameras receive light from the environment and transfer it to 2D image data. Unlike, normal cameras, stereo cameras consist of two or more lenses, providing the ability to reconstruct the three-dimensional world with 2D images. However, cameras are sensitive to variations in illumination and weather conditions and may yield poor images in dark or rainy environments. Unlike passive cameras, LiDARs are less sensitive to illumination and these weather conditions as they are active sensors that can emit and receive reflective infrared light. In addition, LiDARs can provide 3D data with depth information. Camera and LiDAR fusion is garnering more interest due to it can leverage both the depth information from point clouds and color information from 2D images \cite{TSF-FCN}. Radars are another type of active sensors that are also used in autonomous cars. They emit radio waves instead of infrared light waves. While they can detect objects at longer distances, their accuracy is lower compared to LiDARs.  GPS sensors are another type that is vastly used in such vehicles.   GPS provides global location information, which is combined with local information provided by the inertial measurement unit (IMU) to localize the ego-vehicle.

%\begin{figure}[htbp]
%    \centering
%    \includegraphics[width=0.45\textwidth]{figures/self_driving_system.png}
%    \caption{Typical self-driving system with different kinds of sensors}
%    \label{fig:self-driving system}
%\end{figure}


 Different self-driving systems employ various sensor combinations. For instance, Boss won the 2007 DARPA Urban Challenge using eleven LiDARs, five radars, and two cameras. IARA, the first Brazilian self-driving car, operates autonomously using LiDARs and cameras. Waymo, Google's self-driving car, uses multiple radars, LiDARs, and cameras. Apollo integrates LiDARs in its system, while Tesla aims for a camera-only self-driving system by removing radar and ultrasonic sensors. All the aforementioned sensor configurations are summarized in TABLE \ref{tab:sensors settings}.

\begin{table}[ht]
    \centering
        \caption{Sensor settings of different self-driving systems}
    \begin{tabular}{c|c|c|c|c|c}
    \hline
    \textbf{System}  &  \textbf{Camera} & \textbf{LiDAR} & \textbf{Radar} & \textbf{GPS} & \textbf{IMU} \\ \hline
     Boss \cite{Urmson2008AutonomousDI}    &  2  & 11 & 5 & \checkmark & \checkmark \\ 
      IARA \cite{Badue2019SelfDrivingCA}     & 3 & 2 & - & \checkmark & \checkmark    \\ 
     Waymo \cite{Waymo}     & 9   & 4 & 6 & \checkmark & \checkmark    \\ 
     Apollo \cite{Apollo} & 2    & 4 & 2   & \checkmark & \checkmark       \\ 
     Tesla \cite{TeslaAutopilot2023} & 8    & - & -  & \checkmark & \checkmark    \\  \hline
     \end{tabular}
    \vspace{0.2cm}

    \label{tab:sensors settings}
    \vspace{-0.5 cm}
\end{table}





==> x04_Test_and_Evaluation.tex <==
\section{Testing and Evaluating}
%\textit{PASCAL Visual Object Classes (VOC)} projects, particularly the VOC2007 and VOC2012, are well-known datasets and challenges for object detection, semantic segmentation, and image classification. They contain 20 predefined class images, including vehicles, bicycles, animals, etc, and each image has been annotated with information such as the belonging objects for classification, bound box coordinates for object detection, and pixel-level details for segmentation. It also provides evaluation standards, such as average average precision, to facilitate the comparison between different models. The object detection models, such as YOLO \cite{YOLO, Redmon2018YOLOv3AI, Redmon2016YOLO9000BF}, Faster R-CNN \cite{Ren2015FasterRCNN}, and SSD \cite{Liu2015SSDSS} are applied in this dataset to train and evaluate their performance. In addition, Mask R-CNN \cite{matterport_maskrcnn_2017}, aimed at semantic segmentation is also trained and evaluated by this dataset.

Before deploying self-driving systems, whether they are generic modular systems or end-to-end systems, it is imperative that these systems undergo rigorous training and pretest processes. Training involves feeding the machine-learning (ML) models with labeled data from comprehensive datasets, enabling them to learn and adapt to various driving conditions and scenarios. After the models are trained, validation and testing should be deployed to evaluate their performance and reliability by using the simulator and dataset. 

For the generic modular systems, the complex self-driving problem is divided into distinct tasks (see section \ref{se:software systems}). Each module focuses on a specific function and can be trained independently with input tailored to its specific role. The most common types of training inputs for these modules are images and point clouds, which capture the environment in 2D and 3D forms respectively. Regarding training image-based models, there are various datasets available, thanks to the advancements in computer vision. \textit{PASCAL Visual Object Classes (VOC)} project \cite{Everingham2010ThePV}, particularly the VOC2007 and VOC2012, are well-known datasets and challenges for object detection, semantic segmentation, and image classification. They contain 20 predefined class images, including vehicles, bicycles, animals, etc, and each image has been annotated with information such as the belonging objects for classification, bound box coordinates for object detection, and pixel-level details for segmentation. Models, such as YOLO \cite{YOLO, Redmon2018YOLOv3AI, Redmon2016YOLO9000BF}, Faster R-CNN \cite{Ren2015FasterRCNN}, and SSD \cite{Liu2015SSDSS}, are applied in this dataset to train and evaluate their performance. \textit{ImageNet} \cite{Deng2009ImageNetAL}, \textit{COCO} \cite{Lin2014MicrosoftCC}, and \textit{CIFAR-10} and \textit{CIFAR-100} \cite{Krizhevsky2009LearningML} are also the dataset commonly used in computer vision, which can be used to trained the vison modules in the self-driving systems. \textit{Cityscapes} \cite{Cordts2016TheCD} dataset includes video sequences of street scenes from 50 different cities featuring both fine and coarse annotations. This dataset is invaluable for training the vision system of automated driving systems, specifically for the segmentation tasks.

As LiDAR becomes increasingly integrated into self-driving systems, a variety of datasets have been developed to provide the necessary 3D point cloud data for training and validating these systems. In addition, generic image datasets often fall short of capturing the complex scenarios encountered in autonomous driving. Consequently, more datasets specifically tailored to self-driving challenges are proposed. These datasets include both 2D images and 3D point clouds, offering a comprehensive suite to train the models of self-driving systems. \textit{Karlsruhe Institute of Technology and Toyota Technological Institute (KITTI)} \cite{Geisberger2012ExactRI} is a popular dataset for self-driving, especially focusing on 3D object detection and 3D tracking. The data are captured from an ego-vehicle which contains a LiDAR, two stereo cameras, and a GPS. The KITTI dataset is captured from both the rural areas and highways of the city of Karlsruhe. It contains both the LiDAR point clouds and the camera images, enabling the training and evaluation of LiDAR-based algorithms, such as VoxelNet \cite{VoxelNet} and PointPillar \cite{Lang2018PointPillarsFE}, and LiDAR-Camera fusion algorithms, such as MV3D \cite{MV3D} and AVOD \cite{AVOD} based on that. \textit{Waymo open dataset} includes both a perception dataset \cite{Sun2019ScalabilityIP} and a motion dataset \cite{Ettinger2021LargeSI, Chen2023WOMDLiDARRS}. The perception data, rich with high-resolution camera and LiDAR data, provides detailed label information, such as bounding boxes and segmentation labels, making it ideal for training and validating models focused on perception, such as object detection and segmentation. Meanwhile, the motion dataset caters to dynamic object information, such as vehicles, pedestrians, and cyclists, providing tracking IDs, labels, and bound boxes that are generated by models trained on the perception dataset. In addition, the motion dataset contains map information of six cities, enhancing the utility for developing and validating self-driving systems in diverse urban environments. 

Platforms integrated dataset and simulator have been launched to facilitate the deployment of self-driving systems. \textit{Apollo} \cite{Apollo} and \textit{Autoware} \cite{autowarefoundation} serve as generic modular platforms, providing full-stack frameworks for development. Specifically,  \textit{Apollo} \cite{Apollo}, developed by Baidu, offers a data set called, \textit{ApolloScape} \cite{Wang2018TheAO}, which boasts richer label information compared with KITTI \cite{Geisberger2012ExactRI} and Cityscapes \cite{Cordts2016TheCD}. Additionally,  \textit{Apollo} includes a visualization and simulation tool, \textit{Dreamview}, which enhances user interaction with various modules, allowing for the deployment of pre-trained models. \textit{Autoware} \cite{autowarefoundation} comprises of various software modules for self-driving. It also can be integrated with an LGSVL simulator \cite{rong2020lgsvl} to validate the model deployment. Training the end-to-end system is complex, requiring datasets or simulators that provide near-realistic, dynamic scenarios along with the capabilities to simulate various sensors like cameras and Lidar. \textit{Car Learning to Act (CARLA)} \cite{Dosovitskiy17} is an open-source simulator for autonomous driving in urban environments. It can be deployed to train and evaluate the models for self-driving, including perception and control algorithms. CARLA also provides diverse kinds of city layouts and different kinds of vehicles and buildings, etc. The simulator provides different environmental conditions, weather and time, and different sensor suites. According to the setup, the models can be trained and validated within this simulator. Three self-driving approaches are evaluated in \cite{Dosovitskiy17}, including generic modular pipeline, end-to-end imitation learning, and end-to-end reinforcement learning. In addition, two transformer-based imitation learning models, TransFuser \cite{Chitta2022TransFuserIW} and InterFuser \cite{Shao2022SafetyEnhancedAD}, are also based on CARLA.

